Embedding Graph Convolutional Networks in Recurrent Neural Networks for Predictive Monitoring

Predictive monitoring of business processes is a subfield of process mining that aims to predict, among other things, the characteristics of the next event or the sequence of next events. Although multiple approaches based on deep learning have been proposed, mainly recurrent neural networks and convolutional neural networks, none of them really exploit the structural information available in process models. This paper proposes an approach based on graph convolutional networks and recurrent neural networks that uses information directly from the process model. An experimental evaluation on real-life event logs shows that our approach is more consistent and outperforms the current state-of-the-art approaches.

==> Embedding Graph Convolutional Networks in Recurrent Neural Networks for Predictive Monitoring/__latexindent_temp.tex <==
Predictive monitoring is a subfield of process mining concerned with forecasting how an ongoing business case is going to unfold in the future~\cite{Maggi2014}. These predictions may involve information such as what will be the next activity or set of activities, when will happen the next event, or how much time is left until the end of the case. Many machine learning techniques have been used to learn a predictive model that aims to forecast these problems, and, in particular, deep learning arises as one of the most prominent sets of techniques used nowadays, due to their good results~\cite{Tax2018}.

==> __latexindent_temp.tex <==
Predictive monitoring is a subfield of process mining concerned with forecasting how an ongoing business case is going to unfold in the future~\cite{Maggi2014}. These predictions may involve information such as what will be the next activity or set of activities, when will happen the next event, or how much time is left until the end of the case. Many machine learning techniques have been used to learn a predictive model that aims to forecast these problems, and, in particular, deep learning arises as one of the most prominent sets of techniques used nowadays, due to their good results~\cite{Tax2018}.
